Efficient Computation of Visibility Polygons

Determining visibility in planar polygons and arrangements is an important subroutine for many algorithms in computational geometry. In this paper, we report on new implementations, and corresponding experimental evaluations, for two established and one novel algorithm for computing visibility polygons. These algorithms will be released to the public shortly, as a new package for the Computational Geometry Algorithms Library (CGAL).

==> Makefile <==
LANGUAGE = en_US
DOCUMENTS = main.pdf
TEXFILES := $(sort $(wildcard *.tex))

PDFLATEX = pdflatex
PDFLATEXFLAGS = -halt-on-error -file-line-error
BIBTEX = bibtex
BIBTEXFLAGS =

#GRAPHICS_STATIC = $(foreach g, \
#	prototyp.pdf, \
#	pics/$g)

GRAPHICS_STATIC =

GRAPHICS_PDF =

GRAPHICS_PDFTEX = $(foreach g, \
	3sat gadget_and gadget_crossing gadget_inverter gadget_multiplexer \
	gadget_or_bb gadget_or_rb gadget_variable needles three_colorability, \
	graphics/$g.pdf_tex)

main.pdf: main.tex \
	abstract.tex \
	introduction.tex \
	preliminaries.tex \
	conclusion.tex \
	bibliography.bib
#	$(GRAPHICS_STATIC) $(GRAPHICS_PDF) $(GRAPHICS_PDFTEX)

.DEFAULT_GOAL = all
.PHONY: all todo spellcheck clean

all: $(DOCUMENTS)

todo:
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		grep -hnT TODO $$texfile || true; \
		grep -hnTo '\\\(todo\|missingfigure\)\(\[.*\]\)\?{.*}' $$texfile | detex || true; \
	done

spellcheck:
	for texfile in $(TEXFILES); do \
		aspell --lang=$(LANGUAGE) check $$texfile; \
	done

$(DOCUMENTS): %.pdf: %.tex
	$(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}
	if grep -e '\citation' -e '\bibdata' -e '\bibstyle' *.aux; then \
		$(BIBTEX) $(BIBTEXFLAGS) $* && $(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}; \
	fi
	$(PDFLATEX) $(PDFLATEXFLAGS) -recorder \\input{$<}
	grep '^OUTPUT ' $*.fls \
		| sed -e 's/^OUTPUT //' \
		| grep -vx $@ \
		| xargs rm
	rm $*.fls
	rm -f $*.bbl $*.blg

%.ps: %.pdf
	pdf2ps -dLanguageLevel=3 $< $@

$(GRAPHICS_PDF): %.pdf: %.svg
	inkscape --without-gui --export-pdf=$*.pdf $*.svg

$(GRAPHICS_PDFTEX): %.pdf_tex: %.svg
	inkscape --without-gui --export-latex --export-pdf=$*.pdf $*.svg

clean:
	rm -f $(DOCUMENTS)
	rm -f *.aux *.bbl *.blg *.log *.out 
#	rm -f $(GRAPHICS_PDF)
#	rm -f $(GRAPHICS_PDFTEX)
#	rm -f $(GRAPHICS_PDFTEX:.pdf_tex=.pdf)


==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

\todo{Alex}

==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}


